Discrete Representations Strengthen Vision Transformer Robustness

Vision Transformer (ViT) is emerging as the state-of-the-art architecture for image recognition. While recent studies suggest that ViTs are more robust than their convolutional counterparts, our experiments find that ViTs trained on ImageNet are overly reliant on local textures and fail to make adequate use of shape information. ViTs thus have difficulties generalizing to out-of-distribution, real-world data. To address this deficiency, we present a simple and effective architecture modification to ViT's input layer by adding discrete tokens produced by a vector-quantized encoder. Different from the standard continuous pixel tokens, discrete tokens are invariant under small perturbations and contain less information individually, which promote ViTs to learn global information that is invariant. Experimental results demonstrate that adding discrete representation on four architecture variants strengthens ViT robustness by up to 12% across seven ImageNet robustness benchmarks while maintaining the performance on ImageNet.

==> 1_intro_old.tex <==
\section{Introduction}

% list of test to run to lu
% make rng
% gave lu codebook, model ftemb checkpoint.
% mostafa attention pointer

%\lu{@lu draft a readable intro}
% what is robust learning and why it is important
Our world is open, diverse, and naturally changing. 
The distributional shift of visual data between training and inference poses a real challenge for generalization of deep learning models.
Ideally, a robust model should exploit semantic features (\eg, structure and shape) while being invariant to the nuisances features that are unstable and easily changing in new environments.
%should be invariant to the nuisances features, which are unstable and easily changing in new environments \citep{achille2018emergence}, while exploiting the underlying features related to the semantic and shape information.
Recently, several works were proposed to measure deep network's robustness on out-of-distribution data such as ImageNet-A~\citep{imagenet-A}, ImageNet-C~\citep{imgnet-C}, Stylized-ImageNet~\citep{stylized-imgnet}, \etc.
%\citep{objectnet, imagenet-A, hendrycks2021many-ImgR, sketch, stylized-imgnet, imgnet-C}
A typical task is to learn a recognition model on the ImageNet dataset~\cite{}, but test the trained model off-the-shelf on a series of out-of-distribution.
Different from adversarial perturbations 
%which are intentionally engineered to attack the models, 
these ImageNet variant datasets approximate natural distribution of real-world images unseen during training where the changes are brought by background, context, viewpoints, and illumination.

%To verify the 
%\citep{objectnet, imagenet-A, hendrycks2021many-ImgR, sketch, stylized-imgnet, imgnet-C}, underscoring the gap between the machine intelligence and human brain.


% intro to ViTs
Vision Transformer (ViT)~\citep{vit} has started to rival Convolutional Neural Networks (CNNs) in many learning tasks. 
In particular, recent works found that ViTs are more robust than CNNs~\citep{ViTRobust,towardsrobust} and generalize favorably on a variety of ImageNet robustness benchmarks. The benefit stems from the architecture design that captures a different inductive bias than CNNs. By virtue of self-attention, ViT learn globally-contextualized representation.


%Vision Transformer (ViT)~\citep{vit}, which interprets an image as a sequence of \textit{tokens}, has demonstrated comparable recognition accuracy on the ImageNet benchmark with smaller computational budgets. 
%In particular, 
%Self-attention is the core globally-contextualized representation
%by virtue of the architectural design to capture in which each image patch is attended to all patches of the same image.

Learning such globally-contextualized representation and the related features is beneficial and the related increase in shape bias improves accuracy and robustness~\citep{stylized-imgnet}.
Although ViTs are powerful enough to learn global features, we find it still primarily relies on local detail (\eg, texture) than utilizing shape or structure of the object. An evidence is that removing position embedding from ViT only leads to a marginal drop (less than 4\%) on ImageNet but a sharp drops on the robustness ImageNet benchmarks. This issue remains when incorporating strong data augmentation and model regularization.


The results suggest existing vision transformer architectures do not make full use of global shape and structure information even though the self-attention is well capable of modeling global context. Our key insight is that the \emph{linear tokenization process of ViT restricts the capability to capture structure information.} ViT can minimize the loss without knowing the order of the tokens.

%However, the position embedding is only circumferential for image recognition. As suggested in~\citep{ViT_pos,ViTRobust}, removing positional embedding leads to a marginal drop ($\sim$4\%) on the ImageNet benchmark. 
%

% Removing the positional embedding from ViT only results in a relative reduction on the ImageNet dataset.
% ViTs tend to rely more on local cues (\eg, texture) than shape structural information. As shown
% However, evidence shows that ViT models do not make good use of the global structure of the input data \citep{ViT_pos,ViTRobust}. 
% After removing the positional information from the ViT, the model's accuracy reduces only 3\% on ImageNet.



%An ideal token for transformer should have two properties: be faithful on the robust features of the data, and encodes information in the order of the tokens.


%Deep neural networks have achieved high performance when tested on i.i.d. data, such as the image classification \citep{imagenet}. However, our world is open and naturally changing, where the distribution for vision data often shifts to out-of-distribution. Out of distribution data decreases the generalization of the state-of-the-art classifiers significantly \citep{objectnet, imagenet-A, hendrycks2021many-ImgR, sketch, stylized-imgnet, imgnet-C}, underscoring the gap between the machine intelligence and human brain. 

% Generalization is the key measurement for the performance of a deep neural network. Governed by empirical risk minimization, d


% work on robustness
% A large body of work studies how to train model in lab and generalize to unseen, shifted distribution. 
% A robust model should be invariant to the nuisances features, which are unstable and easy to change in new environment \citep{achille2018emergence}, while learning robust features such as the semantic and shape information. 


% In addition, existing deep models are trained to use all signals that help minimize the training loss, even if the signal is nuisances and suboptimal.

% To measure the real-world generalization of models that trained in lab, it is thus important to test the models generalization on out-of-distribution data without training on any of the new test distribution \citep{GenInt}. 

% vit, vitreg, deit,
%Model architecture is another major factor for models' generalization and robustness. 
% 


% We desire an input representation that encodes most of the information in the order of the representation between patches, not the individual patch itself, so that vision transformer can attend to global structure more and improve generalization and robustness.
% The linear representation from patches are over-complete, where the model can still optimize the loss even with the absence of the position information.

In this paper, we propose a simple yet novel input layer for vision transformers, where an image patch is represented by a combination of two embeddings of pixel tokens and \emph{discrete tokens}. To be specific, we discretize an image and represent an image patch as a \emph{discrete token} or ``visual word'' in a codebook. Discrete tokens capture important features in a low-dimensional space~\citep{oord2017neural} that preserves shape and structure of the object, thereby promoting the ViT to spare capacity modeling the structure as opposed to local patterns of the object. As discrete tokens lose local details especially for small object, we use the both embeddings as the input to the existing ViT architectures.
%Our new token promote the ViT model to learn the interaction of input tokens and ignore the local pattern, which naturally improves robustness. 
Our approach only change the image patch tokenizer, which is orthogonal all existing approach to improve generalization and robustness, and can be integrated into future variants for vision transformer architectures. 
%and term our model Token Embedding with Duality or TED-ViT. 

%Motivated by the integer token input in language transformer and the advance in discrete generative models, we propose to add integer token as the code representation to the ViT. Just like a language transformer model that process words encoded in integers tokens, our model process image patches encoded in integers tokens. We use the pretrained VQGAN \citep{VQGAN} as the quantized tokenizer to generate the integer code for the given image. VQGAN model can reconstruct the input image from integer code with high quality, with some difference in local detail. In addition, we find that VQGAn encodes most of the input information in the order of the token, not the individual token.
Empirical experiments and visualizations show that combing integer token with continuous token significantly improves generalization accuracy for all seven out-of-distribution ImageNet benchmarks. Just by replacing the input token feature of the state-of-the-art vision transformer, we gain generalization accuracy on ImageNet-Redition by up to 10\%, Stylized-ImaegNet by up to 12\%, ImageNet-Sketch by up to 9\%, and ImageNet-C by up to 7\%. 

To the best of our knowledge, ours is the first work to improve the robustness of vision transformer by introducing discrete token representations. To summarize, the main contributions of this paper are as follows: \emph{(i)} a simple yet novel architectural modification to ViT that improves the robustness of 4 ViT architectures on 7 out-of-distribution ImageNet benchmarks across the board. Unlike other robust methods that are tailed to specific type distributions, our method is generic and yield consistent improvements. \emph{(ii)} We validate the efficacy of method for the challenging case where the models are pretrained on a large dataset ImageNet21k. \emph{(iii)} Our method achieves the new state-of-the-art by on four benchmarks.

%1. Our proposed method offers a way to make the position embedding matter in ViT.
% 2. We design a novel architectural modification to ViT that improves the robustness on 7 out-of-distribution ImageNet benchmarks across the board.  Unlike other methods that are tailed to specific type of robustness, our method is generic and yield consistent improvement on three ViT/MLP architectures and on large training data ImageNet21k.
% 3..
%Unlike other approaches, our method is generic not tailed to 

% good at 3 shape, dataset
% transorrmer, robust, lose shape, we propose new arch, can capture more shape information.

% two represenattion's advantage, 



==> backup_number.tex <==
\begin{table}[t]
\begin{center}
    \centering
    \scriptsize
    \begin{tabular}{l|c|ccc|ccccc}
         \toprule
         CodeBook &  & \multicolumn{8}{c}{Out of Distribution Robustness Test} \\
          Size & ImageNet & Rendition & Stylized & Sketch & ObjectNet & Real & V2 & A & C $\downarrow$ \\
         \midrule  
         1024 & 77.96&	47.27&	22.27&	36.53&	29.14&	83.95&	66.24&	12.45&	56.85 \\
         4096 & 78.35&	47.32&	21.48&	36.55&	29.48&	84.28&	66.56&	13.43&	55.92\\
         8192 & 78.36&	47.78&	22.66&	36.6&	29.74&	84.25&	67.06&	13.24&	55.87\\
         \bottomrule
    \end{tabular}
\end{center}
\caption{The impact of codebook size for robustness. A larger codebook size helps robustness.\lu{change this to a figure}}\label{tab:ablation_codebook}
\end{table}

==> convert.tex <==
|  Stylized-ImageNet   | CNN | ViT | ViT+ CNN Global Features | Discrete ViT|
|----------------------|-----|-----|--------------------------|-------------|
|Fraction of Shape Bias|0.22 | 0.42|        0.3               |  **0.62**       |




|  Model   | ImageNet | Real | Rendition |Stylized| Sketch|ObjectNet|V2|A|C &darr;|
|----------|----------|------|-----------|--------|-------|---------|--|---|-------|
|ViT|78.73 | 84.85 | 38.15 | 10.39 | 28.60 | 28.71 | 67.34 | 16.92 | 53.51 |
|ViT+Global CNN Continuous Feature| 78.51 | 83.44 | 34.66 | 10.47 | 25.14 | 28.35 | 65.86 | 15.97 | 57.64|
ViT + Ours | **79.48** | **84.86** | **44.77** | **19.38** | **34.59**  | **30.55**  | **68.05** | **17.20** | **46.22** |





|  Discrete Tokenization Model   | ImageNet | Real | Rendition |Stylized| Sketch|ObjectNet|V2|A|C &darr;|
|----------|----------|------|-----------|--------|-------|---------|--|---|-------|
|None|78.73 | 84.85 | 38.15 | 10.39 | 28.60 | 28.71 | 67.34 | 16.92 | 53.51 |
|VQ-VAE |78.36 | 84.35 | **46.22** | **23.36** | **35.17** | **29.34** | 66.24 | 13.61 | **52.20** |
VQ-GAN | **79.48** | **84.86** | **44.77** | **19.38** | **34.59**  | **30.55**  | **68.05** | **17.20** | **46.22** |
